Parameter Importance-Driven Continual Learning for Foundation Models

Domain-specific post-training often causes catastrophic forgetting, making foundation models lose their general reasoning ability and limiting their adaptability to dynamic real-world environments. Preserving general capabilities while acquiring downstream domain knowledge is a central challenge for large language and multimodal models. Traditional continual learning methods, such as regularization, replay and architectural isolation, suffer from poor downstream performance, reliance on inaccessible historical data, or additional parameter overhead. While recent parameter-efficient tuning (PET) methods can alleviate forgetting, their effectiveness strongly depends on the choice of parameters and update strategies. In this paper, we introduce PIECE, a Parameter Importance Estimation-based Continual Enhancement method that preserves general ability while efficiently learning domain knowledge without accessing prior training data or increasing model parameters. PIECE selectively updates only 0.1% of core parameters most relevant to new tasks, guided by two importance estimators: PIECE-F based on Fisher Information, and PIECE-S based on a second-order normalization that combines gradient and curvature information. Experiments across three language models and two multimodal models show that PIECE maintains general capabilities and achieves state-of-the-art continual learning performance across diverse downstream tasks. Our results highlight a practical path to scalable, domain-adaptive foundation models without catastrophic forgetting.

==> sec/1_intro-back.tex <==
\section{Introduction}
\label{sec:intro}
% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=0.5\linewidth]{{pic/pic1_result_overview.pdf}
%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pic/pic1_result_overview.pdf}
    \caption{Comparison of continual learning methods on Llama3-8B, showing average task scores after training on the benchmark (top) and changes in original programming ability on HumanEval as training tasks increase (middle: full-parameter baselines; bottom: parameter-efficient baselines), where SPTC consistently outperforms others in both transfer and capability retention.}
    \label{fig:placeholder}
\end{figure}

% 近年来，大语言模型取得了显著进展，在自然语言理解~ref、多模态推理~ref 等任务上实现了突破，广泛应用于医疗、科学等多个领域~ref。然而，现实世界中概念与领域知识的不断演化，对模型的适应能力提出了更高要求。持续学习被认为是一种有效途径~ref，使大语言模型能够通过不断训练吸收新的领域知识。持续学习的关键难题是灾难性遗忘~ref，新任务表现的提升往往伴随着旧任务性能的下降~ref，最终导致整体性能的下降。许多方法被提出来解决持续学习中的灾难性遗忘问题，大致可以按以下进行分类：1、基于正则化的方法~ref，通过设计正则化目标来辅助持续学习期间过去任务学习信息的保留。2、基于回放的方法~ref，通过将新任务训练数据和小部分旧任务数据混合来维持旧任务性能。3、基于架构的方法~ref，通过设计新架构组件来最大限度地减少任务间的干扰。然而基于正则和基于回放的放依赖历史数据相关信息，在大模型背景下这些数据往往是难以获得的~ref。部分基于架构的方法依赖任务标签，这在大模型场景中也是具有挑战或是不可行的~ref。
% 为探究如何在不获取模型预训练数据，不对任务数据进行分类并且不改变模型架构的前提下微调模型进行领域迁移的同时保持模型原能力。我们评估了不同持续学习方法的表现，通过分析我们发现：1、参数高效微调相较于全量微调更能保护模型原能力，如图一所示，由于缺失了原模型训练数据，基于正则和基于回放的方法都导致了原模型能力的灾难性遗忘，而基于参数高效微调的方法都一定程度上缓解了这一问题。2、不同参数高效微调方法的持续学习能力表现不同，微调参数选取差异导致模型在领域迁移效果和原能力保持上都会存在差异。
% 基于这些见解，并受到参数高效微调一些成功的工作的启发，我们提出了SPTC方法，通过关注任务最为相关的参数进行参数高效微调，在不依赖任何历史数据信息的情况下完成持续学习。具体来说，在训练开始前，分别基于Fisher信息量（STPC-F）和二阶归一化方法（SPTC-S）的经验近似来估计每个参数重要性，然后选择最为重要的K个参数作为实现领域迁移的更新参数，冻结其他参数来维持模型整体稳定保护原能力。
% 为验证 SPTC 方法的有效性，我们在大语言模型和多模态大语言模型两类模型上进行了系统而广泛的实验，涵盖从 2B 到 14B 不同规模的模型。实验结果表明，SPTC 方法在跨领域迁移能力和历史知识保持方面均表现出显著优势，尤其在维持模型原有能力方面效果突出，能够在引入新知识的同时有效避免遗忘现象。
% 我们的主要贡献有三个：
% 我们为持续学习引入新的参数高效微调框架SPTC。无需历史训练数据信息，不增加模型参数的情况下应对模型灾难性遗忘挑战
% 为SPTC的参数重要性评价提供基于Fisher信息量和二阶归一化方法的两种方案，并实验分析两者差异及各自优势
% 大语言模型和多模态大语言模型上的丰富实验结果证明了SPTC的显著优越性。



% 近年来，大语言模型在自然语言理解~ref、多模态推理~ref 等任务中取得了显著进展，并已广泛应用于医疗、科学等领域~ref。然而，现实世界中的概念与领域知识不断演化，对模型的适应能力提出了更高要求。持续学习被认为是一种有效途径~ref，使大语言模型能在不断训练中吸收新的领域知识。持续学习面临的核心挑战是灾难性遗忘~ref：新任务性能的提升通常伴随着旧任务性能的下降~ref，从而导致整体性能下降。
In recent years, large language models (LLMs) have achieved remarkable advances in tasks such as natural language understanding~\cite{karanikolas2023large, zhuang2022acil} and multimodal reasoning~\cite{li2025survey, mitra2024compositional}, and have been widely applied in diverse fields including healthcare~\cite{chen2025mimo} and science~\cite{yan2025position}. However, concepts and domain knowledge in dynamic real-world continuously evolve, requiring models to adapt accordingly~\cite{liu2020learning}. Continual learning~\cite{mccloskey1989catastrophic} has been recognized as an effective mechanism for LMs to incrementally acquire new domain knowledge~\cite{shi2024continual}. A main challenge in continual learning is catastrophic forgetting~\cite{french1999catastrophic}: improvements on new tasks often come at the cost of performance degradation on previous tasks, which can lead to an overall decline in model performance.

% 为应对持续学习中的灾难性遗忘问题，已有方法可以大致分为三类：（1）基于正则化的方法~ref：通过设计正则化目标，在持续学习过程中帮助模型保留过去任务的学习信息。（2）基于回放的方法~ref：通过将新任务数据与少量旧任务数据混合训练，以维持旧任务性能。（3）基于架构的方法~ref：通过设计新的架构组件，减少任务间干扰。然而，基于正则化和回放的方法依赖历史数据，这在大模型背景下通常难以获取~ref。部分基于架构的方法依赖任务标签，在大模型场景中同样具有挑战性甚至不可行~ref。
To tackle the catastrophic forgetting problem in continual learning, Numerous approaches have been proposed, which can be broadly classified as follows: (1) \textbf{Regularization-based methods}~\cite{kirkpatrick2017overcoming, chaudhry2019efficient, li2017learning} design regularization objectives to help the model retain knowledge from previous tasks during continual learning; (2) \textbf{Replay-based methods}~\cite{rebuffi2017icarl, rolnick2019experience} mix new task data with a small subset of previous task data to preserve performance on old tasks; and (3) \textbf{Architecture-based methods}~\cite{tong2025analytic, zhao2024sapt} introduce new architectural components to minimize interference between tasks. However, regularization- and replay-based methods rely on access to historical data, which is often difficult to obtain in the context of large models~\cite{touvron2023llama}. 
% Some architecture-based methods also depend on task labels, which can be challenging or even infeasible in large-scale model scenarios~\cite{du2024unlocking}.
Some architecture-based methods isolate tasks by introducing additional model parameters, but such expansion leads to substantial computational and memory overhead in large-scale settings~\cite{verma2021efficient}.

% 为了探究在不依赖预训练数据、不区分任务标签、且不改变模型架构的前提下，如何通过微调实现领域迁移并同时保持模型原有能力，我们首先对多种持续学习方法进行了系统评估，并据此得到以下观察：（1）参数高效微调（Parameter-Efficient Tuning, PET）相比全量微调更能保护模型的原有能力。 如图~\ref{fig1} 所示，由于缺乏原始训练数据，基于正则化和回放的方法均出现了严重的灾难性遗忘，而参数高效微调方法在一定程度上缓解了这一问题。（2）不同参数高效微调方法在持续学习能力上表现存在差异。 不同的参数选择策略会导致模型在领域迁移效果与原有能力保持方面均呈现不同的表现。
To investigate how domain transfer can be achieved through fine-tuning while preserving the original capabilities of models without relying on pretraining data, distinguishing task labels, or modifying the model architecture, we first conducted a systematic evaluation of various continual learning methods. By analyzing the limited of existing methods, we find that: (1) \textbf{Parameter-Efficient Tuning (PET) better preserves the original capabilities of the model compared to full fine-tuning}: as shown in Fig.~\ref{fig:placeholder}, due to the lack of access to original training data, both regularization- and replay-based methods suffer from severe catastrophic forgetting, whereas PET methods alleviate this issue to some extent. 
% (2) \textbf{Different PET strategies exhibit varying performance in continual learning}:
(2) \textbf{Parameter-efficient tuning strategies targeting different adaptation objectives show distinct effectiveness in continual learning scenarios}:
the choice of parameters to fine-tune significantly affects both domain transfer effectiveness and preservation of the model’s original capabilities.

% 基于上述观察，并受到参数高效微调（PET）方法成功实践的启发，我们提出了一种新的参数高效持续学习方法——SPTC。该方法通过关注与当前任务最相关的参数，实现了在不依赖历史数据的前提下的持续学习。具体而言，SPTC在训练前基于两种独立策略评估参数重要性：一种基于 Fisher 信息量（SPTC-F）的经验近似，用于衡量参数对当前任务损失的敏感性；另一种为二阶归一化方法（SPTC-S），通过梯度与二阶曲率信息的经验近似结合来刻画参数的重要程度。随后，选择最重要的 $K$ 个参数进行更新，并冻结其余参数，从而在实现有效领域迁移的同时保持模型原有能力。
Building on these insights and inspired by the success of parameter-efficient tuning (PET) methods~\cite{sung2021training, xu2021raise}, we propose a novel PET-based continual learning approach, SPTC. This method focuses on the parameters most relevant to the current task, enabling continual learning without relying on historical data. Specifically, before training, SPTC evaluates parameter importance using two independent strategies: one is an empirical approximation based on Fisher information (SPTC-F), which measures the sensitivity of parameters to the current task loss; the other is a second-order normalized method (SPTC-S), which uses empirically estimated gradients and second-order curvature information to assess parameter importance. Based on these importance scores, the top-$K$ parameters are updated during training, while the remaining parameters are frozen, enabling effective domain transfer while preserving the model’s original capabilities.

% 为验证 SPTC 方法的有效性，我们在大语言模型（LLMs）和多模态大语言模型（MLMs）两类模型上进行了系统且广泛的实验，涵盖从 2B 到 14B 不同参数量规模的模型。实验结果表明，SPTC 在跨领域迁移能力和历史知识保持方面均表现出显著优势，尤其在维持模型原有能力方面表现突出，能够在引入新知识的同时有效缓解遗忘现象。
We conducted extensive experiments on both large language models (LLMs) and multimodal large language models (MLLMs), covering model scales from 2B to 14B parameters. The results demonstrate that SPTC achieves significant advantages in both cross-domain transfer and preservation of prior knowledge. In particular, it excels at maintaining the original capabilities of the model, effectively mitigating catastrophic forgetting while incorporating new knowledge.

% 我们的主要贡献有三个：
% （1） 提出了一个面向持续学习的新型参数高效微调框架 SPTC，在无需历史训练数据且不增加模型参数的条件下，有效应对大模型的灾难性遗忘问题。
% （2） 针对参数重要性评估，考虑了基于 Fisher 信息量（SPTC-F）和二阶归一化方法（SPTC-S）的两种独立策略，并通过实验分析了它们的差异与各自优势。
% （3） 在多种大语言模型（LLMs）与多模态大语言模型（MLMs）上的实验验证了 SPTC 的显著优越性，尤其在保持模型原有能力方面效果突出。
Our contributions can be summarized as follows:

\begin{itemize}
    \item We introduce SPTC, a parameter-efficient tuning framework for continual learning that mitigates catastrophic forgetting in large models without requiring historical training data or additional parameters.
    
    \item We consider two independent strategies for parameter importance assessment: Fisher information (SPTC-F) and a second-order normalized method (SPTC-S), and analyze their differences and respective advantages.
    
    \item Extensive experiments on various large language models (LLMs) and multimodal large language models (MLLMs) demonstrate SPTC’s effectiveness, particularly in preserving the models’ original capabilities.
\end{itemize}

==> sec/4_experiment-back.tex <==
\section{Experiments}
\label{sec:experiments}
% 我们在多个基准数据集上，选取了各类持续学习基线方法进行对比，以验证我们方法的有效性。实验涵盖了语言和多模态任务，并参考了各自领域近期研究的标准实验设置~\cite{}。
We validate our method on several benchmark datasets against a variety of continual learning baselines. The experiments cover both language and multimodal tasks, and follow the experiment setups in recent works for each respective field~\cite{}
\subsection{Experiment Setup}
\textbf{Datasets}
% 为评估方法在语言任务上的性能，我们在TRACE基准数据集上对所提方法进行了验证。该数据集涵盖八个子集，涉及科学、金融、社会新闻等多个领域，包含英语、德语、中文等多种语言，并引入了代码问题与数学推理等复杂任务。我们采用每个任务包含1000个训练样本的数据集进行实验，各任务具体信息详见补充材料A。此外，鉴于编程能力被普遍认为是模型后训练中易遗忘的代表性先验知识~\cite{}，我们将其作为模型原能力保护的指标并通过Humaneval~\cite{}基准进行量化。
To evaluate our method's performance on language tasks, we conduct experiments on the TRACE~\cite{} benchmark. The benchmark consists of eight sub-datasets covering domains like science (Sin.), finance (Fom.), and social news (Mee.). It covers multiple languages including English, German (20M.), and Chinese (Cst.), and incorporates complex tasks such as code question (Py150) and mathematical reasoning (Ngc, Ngd). We use the version containing 1,000 training samples per task. Detailed information on each task is provided in supplementary materials A. Furthermore, since programming capability is widely recognized as an ability that is prone to forgotting during post-training~\cite{}, we employ it to assess the retention of the model's general capabilities, use the HumanEval~\cite{} benchmark to quantify.
% 为评估方法在多模态任务上的表现，我们在VQA v2基准上延续VQACL与CL-MoE的设置，将数据按问题类别划分为多个任务，每类随机采样1000个训练样本并保留原测试集。我们选择了相较VQA任务标签语义输出更为丰富的图片描述任务作为模型原能力变化评估任务通过flickr30k~\cite{}测试基准进行量化。
% 为评估方法在多模态任务上的表现，我们在VQA v2基准上进行了持续学习实验并选择了相较VQA任务标签语义输出更为丰富的图片描述任务作为模型原能力变化评估任务，通过flickr30k~\cite{}测试基准进行量化。延续VQACL与CL-MoE的设置，将数据按问题类别划分为多个任务，每类随机采样1000个训练样本并保留原测试集，并最终选取下游任务训练效果较好且会对模型图片描述能力造成较大影响的三个任务：action(act.), commonsense(com) and count(cou.)
To evaluate our method's performance on language tasks, we conduct experiments on the  VQA v2~\cite{} benchmark. Following the VQACL~\cite{} setup, we divide the VQA v2 into different tasks based on question types and randomly select 1,000 training samples per task while retaining the original test set. Based on the new task performance improvement and the degree of impairment to the model's original capabilities, three task categories were ultimately selected: action (act.), commonsense (com.), and count (cou.). \\
% 我们将PIECE方法与多种类型的持续学习基线进行了比较：
% \begin{itemize}
%     \item Regularization-based methods:EWC通过参数重要性计算惩罚项，约束重要参数的更新；GEM利用旧任务样本的梯度信息，将参数更新投影到不增加旧任务损失的方向；LwF通过知识蒸馏损失作为正则项，使当前模型输出逼近旧模型输出。
%     \item Replay-based methods:该类方法通过重复利用历史数据来缓解遗忘。本文考虑了两种典型范式：Replay在新任务训练结束后，统一对历史任务数据进行回放学习；Replay-online在训练新任务过程中，持续将历史数据与新任务数据混合学习。以上方法均使用真实数据作为回放数据。
%     \item Architecture-based methods: 本文重点关注基于参数高效微调的基线。SeqLoRA在共享的同一组LoRA参数上顺序执行多个任务的训练；O-LoRA以不同任务的LoRA子空间正交为目标分别优化参数，并在测试阶段将所有LoRA权重相加；LayerNorm仅更新模型中的layernorm部分参数，保持其余参数冻结；MIGU作为一种非结构化参数高效微调方案，依据线性层输出幅度的大小来衡量参数重要性，并据此指导更新。
% \end{itemize}
% 此外，我们还进行了顺序任务下的全量微调（SeqFT）。
\textbf{Baselines} We compared the PIECE method with various types of continual learning baselines:
\begin{itemize}
    \item Regularization-based methods: EWC~\cite{} calculates a penalty term based on parameter importance to constrain updates to important parameters; GEM~\cite{} uses gradient information from old task samples to project parameter updates in a direction that does not increase the old task's loss; LwF~\cite{} uses knowledge distillation loss as a regularizer to make the current model's output approach the output of the old model.
    \item Replay-based methods: This class of methods mitigates forgetting by repeatedly using historical data. We consider two typical paradigms: Replay, which replays historical task data after training a new task~\cite{rebuffi2017icarl}; and Replay-online, which continuously mixes historical data with new task data during training~\cite{rolnick2019experience}. All of these methods use real data for replay.
    \item Architecture-based methods: This paper focuses on baselines based on parameter-efficient fine-tuning. SeqLoRA~\cite{} sequentially trains multiple tasks on a shared set of LoRA parameters; O-LoRA~\cite{} optimizes parameters by targeting orthogonality across LoRA subspaces for different tasks, and at the test stage, it sums all LoRA weights; LayerNorm~\cite{} only updates the layernorm parameters of the model, keeping the other parameters frozen; MIGU~\cite{}, as an unstructured parameter-efficient fine-tuning method, measures parameter importance based on the magnitude of the linear layer's output and uses this to guide updates.
\end{itemize}
Additionally, we performed full fine-tuning (SeqFT) under sequential tasks. \\
% \textbf{Models and Implementation Details} We use the following models for task learning: Gemma2-2B\footnote{https://huggingface.co/google/gemma-2-2b-it}~\cite{gemma_2024}, Llama3-8B\footnote{https://huggingface.co/meta-llama/Meta-Llama-3-8B}~\cite{llama3modelcard}, and Qwen3-14B\footnote{https://huggingface.co/Qwen/Qwen3-14B}~\cite{qwen3technicalreport} for language tasks. Qwen3-VL-4B\footnote{https://huggingface.co/Qwen/Qwen3-VL-4B-Instruct}~\cite{qwen3technicalreport} and LLaVA-1.5-7B\footnote{https://huggingface.co/llava-hf/llava-1.5-7b-hf}~\cite{liu2023visual, liu2024improved} for multimodal tasks. The order of the language tasks is largely consistent with that in TRACE, except that the Py150 task is placed at the end to control the influence on the model's intrinsic capabilities. The multimodal tasks are arranged in order of their impact on the model's original capabilities, with the sequence being: action, commensense, and count. All models are trained using the Adam optimizer, with a batch size of 64 and a random seed set to 42. The learning rates are set as follows: for Gemma2-2B, the learning rates for LoRA and O-LoRA are 5e-4, and 5e-5 for the other methods; for the other models, the learning rates for LoRA and O-LoRA are 1e-4, and 1e-5 for the remaining methods. No warmup strategy is used for any of the tasks. The Qwen3-14B model is trained for 1 epoch per task, while the other models are trained for 5 epochs per task. The experiments in this paper are conducted on 4 x 80G A100 GPUs, 4 x 80G A6000 GPUs, and 8 x 40G A100 GPUs. Details regarding the special deployment of different baselines can be found in Supplementary Material B. \\
\textbf{Models and Implementation Details} We use the following models for task learning: Gemma2-2B~\cite{gemma_2024}, Llama3-8B~\cite{llama3modelcard}, and Qwen3-14B~\cite{qwen3technicalreport} for language tasks. Qwen3-VL-4B~\cite{qwen3technicalreport} and LLaVA-1.5-7B~\cite{liu2023visual, liu2024improved} for multimodal tasks. The order of the language tasks is largely consistent with that in TRACE, except that the Py150 task is placed at the end to control the influence on the model's intrinsic capabilities. The multimodal tasks are arranged in order of their impact on the model's original capabilities, with the sequence being: action, commensense, and count. All models are trained using the Adam optimizer, with a batch size of 64 and a random seed set to 42. The learning rates are set as follows: for Gemma2-2B, the learning rates for LoRA and O-LoRA are 5e-4, and 5e-5 for the other methods; for the other models, the learning rates for LoRA and O-LoRA are 1e-4, and 1e-5 for the remaining methods. No warmup strategy is used for any of the tasks. The Qwen3-14B model is trained for 1 epoch per task, while the other models are trained for 5 epochs per task. The experiments in this paper are conducted on 4 x 80G A100 GPUs, 4 x 80G A6000 GPUs, and 8 x 40G A100 GPUs. Details regarding the special deployment of different baselines can be found in Supplementary Material B. \\
% 我们使用Gemma2-2B~\cite{}\footnote{}, Llama3-8B~\cite{}\footnote{} 和Qwen3-14B作为语言模型来学习语言任务，使用Qwen3-VL-4B~\cite{}\footnote{}和LLaVA-1.5-7B作为多模态模型来学习多模态任务。语言任务的顺序和TRACE中的顺序基本一致，不同的是将任务Py150放到最后来控制对原模型待测能力的影响。多模态任务的顺序则是按照对模型原能力影响程度从小到大进行安排，具体为action，commensense，count。所有模型所有方法所有任务均使用Adam优化器，具体使用的学习率为：Gemma2-2B模型lora和o-lora学习率设置为5-e4,其余方法方法学习率设置为5e-5,另外模型的lora和o-lora方法学习率设置为1e-4，其余方法则设置为1e-5，所有模型所有任务均不设置warmup。除Qwen3-14B模型每个任务训练1轮外，其余模型的每个任务均训练5轮，所有模型的所有任务batch_size均设置为64。所有随机种子均设置为42。本文实验在4张80G A100,4张80G A6000和8张40G A100上完成。其余有关不同baseline的特殊部署细节可在补充材料B中获取。
% 我们使用以下模型进行任务学习：Gemma2-2B~\cite{}\footnote{}、Llama3-8B~\cite{}\footnote{} 和Qwen3-14B用于语言任务，Qwen3-VL-4B~\cite{}\footnote{} 和LLaVA-1.5-7B用于多模态任务。语言任务的顺序与TRACE中的安排大致相同，不同的是将Py150任务放在最后，以控制对模型原始能力的影响。多模态任务则按照对模型原始能力影响的大小依次排列，顺序为：action、commensense 和 count。
% 所有模型使用Adam优化器进行训练，batch_size均设置为64，随机种子设置为42。学习率的设置如下：Gemma2-2B的LoRA和O-LoRA方法为5e-4，其余方法为5e-5；其他模型的LoRA和O-LoRA方法为1e-4，其余方法为1e-5。所有任务均不使用warmup策略。Qwen3-14B模型在每个任务上训练1轮，其余模型每个任务训练5轮。本文实验在4张80G A100,4张80G A6000和8张40G A100上完成。关于不同基线的特殊部署细节，请参见补充材料B。
% 设定在完成任务t后，模型在任务i上的表现评分为R_t,i。对于分类任务或标签为单个token的问答任务，表现评分采用准确率；而对于其他任务，表现评分则为Rouge-L和Bleu分数的均值。我们使用以下指标来衡量不同方法在顺序任务中的学习效果：
% overall performance(OP):衡量在任务t训练结束后，模型对所有已学任务的综合表现：
% backward transfer（BWT）：衡量后续任务的学习对所学任务的表现的影响程度：
% 上述指标仅在顺序任务上进行计算，以便更好地将我们的方法与其他基线方法进行对比，并单独评估模型原始能力的变化：
% 语言模型在Humaneval数据集上测试其代码编程能力，采用Pass@K作为评估指标，
% \begin{equation}\mathrm{Pass@K}=\frac{1}{N}\sum_{i=1}^{N}\mathbb{I}(y_{i}\in\{\hat{y}_{i}^{(1)},\hat{y}_{i}^{(2)},\ldots,\hat{y}_{i}^{(K)}\})\end{equation}
% 其中y_i表示通过测试用例的代码，\hat{y}_{i}^{(k)表示第k个推理结果，本文中 k 设置为1，以衡量模型在单次尝试中生成正确代码的能力。
% 多模态模型使用flickr30k数据集测试模型图片描述能力，使用Rouge-L和Bleu的均值作为指标。
\textbf{Metrics} Let the performance score of the model on task \(i\) after learning task \(t\) be denoted as \(R_{t,i}\). For classification tasks or question-answering tasks with single-token labels, the performance score is measured by accuracy; for other tasks, the performance score is the average of the Rouge-L and BLEU scores. We use the following metrics to assess the learning effects of different methods on sequential tasks:
\begin{itemize}
    \item Overall performance (OP)~\cite{}: Measures the model's overall performance on all learned tasks after training on the task \(t\): 
    \begin{equation}OP_t=\frac{1}{t}\sum_{i=1}^tR_{t,i}\end{equation}
    \item Backward Transfer (BWT)~\cite{}: Measures how much the learning of subsequent tasks influences the performance of a learned task: 
    \begin{equation}BWT_t=\frac{1}{t}\sum_{i=1}^{t-1}\left(R_{t,i}-R_{i,i}\right)\end{equation}
\end{itemize}
The above metrics are calculated only on sequential tasks to better compare our method with other baseline methods, and to separately evaluate the changes in the model's original capabilities:
\begin{itemize}
    \item The language model is tested on the Humaneval dataset to evaluate its code generation ability, using Pass@K as the evaluation metric: 
    \begin{equation}\mathrm{Pass@K}=\frac{1}{N}\sum_{i=1}^{N}\mathbb{I}(y_{i}\in\{\hat{y}_{i}^{(1)},\hat{y}_{i}^{(2)},\ldots,\hat{y}_{i}^{(K)}\}), \end{equation}
    where \(y_i\) represents the correct code for the \(i\)-th test case, and \(\hat{y}_{i}^{(k)}\) represents the \(k\)-th inference result for the \(i\)-th test case. In this paper, \(K\) is set to 1, to evaluate the model's ability to generate correct code in a single attempt.
    \item The multimodal models are evaluated on the Flickr30K dataset to test their image captioning ability, using the average of Rouge-L and BLEU scores as the metric. 
\end{itemize}
\subsection{Results and Analysis}

\begin{table*}[!t]
\centering
% \resizebox{0.98\textwidth}{!}{
\setlength{\tabcolsep}{1.4mm}{
\begin{tabular}{lccccccccccc}
\hlineB{4}
% \multirow{2}{*}{Methods} & \multicolumn{10}{c}{Various task in VQA v2} & \multirow{2}{*}{$AP(\uparrow)$} & \multicolumn{1}{l}{\multirow{2}{*}{$AF(\downarrow)$}} \\ \cline{2-9}
% &  C-S & FOMC & MB & SQA & NGcm & NGds & 20M & Py150 &  & \multicolumn{1}{l}{} \\ \hline
% \multicolumn{13}{l}{\emph{VL-T5}} \\ \hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{HumanEval$(\uparrow)$} & \multicolumn{8}{c}{Various task in TRACE $(\uparrow)$} & \multirow{2}{*}{$OP(\uparrow)$} & \multirow{2}{*}{$BWT(\uparrow)$} \\ 
\cline{3-10}& & Cst. & Fom. & Mee. & Sin. & Ngc. & Ngd. & 20M. & Py150 &  \\ \hline
\multicolumn{12}{l}{\emph{Gemma2-2B}} \\ \hline
SeqFT  & 0.0 & 23.70 & 0.0 & 7.28 & 1.65 & 7.40 & 38.77 & 2.91 & 39.35 & 15.13 & -19.08 \\
EWC & 0.0 & 21.25 & 18.95 & 5.36 & 3.50 & 2.47 & 39.69 & 3.21 & 42.65 & 17.13 & -13.99 \\
GEM & 0.0 & 32.95 & 13.51 & 4.50 & 16.20 & 6.17 & 35.69 & 2.86 & 41.31 & 19.15 & -16.27 \\
LwF & 0.0 & 10.15 & 11.41 & 11.64 & 10.01 & 17.41 & 39.69 & 10.24 & 14.33 & 16.86 & -10.10 \\
replay & 0.0 & 33.40 & 37.09 & 17.19 & 43.15 & 3.70 & 32.62 & 7.96 & 34.01 & 26.14 & \underline{-1.43} \\
replay-online & 0.0 & 33.10 & 40.52 & \underline{18.52} & 44.45 & 13.58 & 34.77 & 8.53 & 39.35 & 29.10 & -3.82 \\
SeqLoRA & 10.37 & 45.75 & 35.28 & 11.31 & 67.25 & \textbf{38.27} & \underline{50.77} & 12.18 & \textbf{57.36} & 39.77 & -10.80 \\
O-LoRA & 13.41 & 48.85 & \textbf{57.26} & 16.24 & 72.00 & 33.33 & \textbf{51.38} & 11.57 & 54.55 & \underline{43.15} & -3.45 \\
LayerNorm & 21.95 & 52.75 & 35.28 & 8.65 & 75.75 & 12.35 & 9.54 & 9.78 & 13.78 & 27.23 & -1.67 \\
MIGU & 1.22 & 35.00 & 4.64 & 9.46 & 16.00 & 12.35 & 42.77 & 8.33 & 53.12 & 22.71 & -10.36 \\
SPTC-F (ours) & \underline{32.32} & \underline{53.10} & \underline{53.43} & 18.17 & \textbf{76.25} & \underline{34.57} & \underline{50.77} & \textbf{12.90} & \underline{55.48} & \textbf{44.33} & -3.21 \\
SPTC-S (ours) & \textbf{33.54} & \textbf{54.35} & 52.22 & \textbf{19.37} & \underline{75.85} & 22.22 & 45.23 & \underline{12.75} & 54.24 & 42.03 & \textbf{-1.18} \\
\hline
\multicolumn{12}{l}{\emph{Llama3-8B}} \\ \hline
SeqFT  & 0.0 & 47.10 & 58.67 & 23.77 & 41.75 & 28.40 & 47.70 & 13.32 & 53.05 & 39.22 & -10.69 \\
EWC & 0.0 & 33.95 & 58.67 & 22.10 & 21.20 & 27.16 & 39.08 & 11.33 & 50.13 & 32.95 & -10.05 \\
GEM & 0.0 & 41.05 & \underline{60.48} & 24.33 & 47.75 & 27.16 & 48.92 & 10.80 & 54.43 & 39.37 & -10.24\\
LwF & 0.0 & 39.80 & 44.07 & 12.14 & 40.20 & 23.45 & 49.23 & 10.67 & 44.92 & 33.06 & -9.94\\
replay & 0.0 & 42.45 & \underline{60.48} & \underline{25.88} & 53.55 & 25.93 & 40.62 & 11.20 & 48.84 & 38.62 & -2.94\\
replay-online & 0.0 & \textbf{52.25} & \textbf{65.32} & \textbf{26.46} & \underline{76.95} & 38.27 & 42.46 & 10.78 & 51.25 & 45.47 & -1.99\\
SeqLoRA & 28.05 & 47.15 & 56.05 & 18.62 & 72.75 & 54.32 & \textbf{53.23} & 12.51 & 53.67 & 46.04 & -4.39 \\
O-LoRA & 26.83 & 45.20 & 39.52 & 17.57 & 61.30 & 43.20 & 48.00 & 11.73 & 51.30 & 39.73 & -7.19\\
LayerNorm & 27.44 & 34.90 & 27.02 & 9.44 & 66.80 & 37.04 & 35.08 & 9.34 & 23.50 & 30.39 & \underline{-1.86}\\
MIGU & 0.0 & 38.60 & 25.40 & 20.93 & 59.35 & 41.98 & 49.23 & 11.42 & 54.29 & 37.65 & -10.02\\
SPTC-F (ours) & \underline{29.88} & 47.95 & 59.88 & 23.42 & 76.40 & \textbf{61.73} & \textbf{57.85} & \underline{13.50} & \textbf{59.65} & \textbf{50.05} & -2.64\\
SPTC-S (ours) & \textbf{32.32} & \underline{49.05} & 57.66 & 23.47 & \textbf{77.10} & \underline{59.26} & 52.62 & \textbf{14.00} & \underline{59.24} & \underline{49.05} & \textbf{-1.78}\\
\hline
\multicolumn{12}{l}{\emph{Qwen3-14B}} \\ \hline
SeqFT  & 0.0 & 47.10 & 58.67 & 23.77 & 41.75 & 28.40 & 47.70 & 13.32 & 53.05 & 39.22 & -10.69 \\
EWC & - & 33.95 & 58.67 & 22.10 & 21.20 & 27.16 & 39.08 & 11.33 & 50.13 & 32.95 & -10.05 \\
GEM \\
LwF \\
replay \\
replay-online \\
SeqLoRA \\
O-LoRA \\
LayerNorm \\
MIGU \\
SPTC-F (ours) \\
SPTC-S (ours) \\
\hlineB{4}
\end{tabular}}
\caption{Language Model}
\label{tab1}
\end{table*}

\begin{table}[!t]
\centering
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1.4mm}{
\begin{tabular}{lcccccc}
\hlineB{4}
% \multirow{2}{*}{Methods} & \multicolumn{10}{c}{Various task in VQA v2} & \multirow{2}{*}{$AP(\uparrow)$} & \multicolumn{1}{l}{\multirow{2}{*}{$AF(\downarrow)$}} \\ \cline{2-9}
% &  C-S & FOMC & MB & SQA & NGcm & NGds & 20M & Py150 &  & \multicolumn{1}{l}{} \\ \hline
% \multicolumn{13}{l}{\emph{VL-T5}} \\ \hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{flickr30k} & \multicolumn{3}{c}{Various task in VQA} & \multirow{2}{*}{$OP(\uparrow)$} & \multirow{2}{*}{$BWT(\uparrow)$} \\ 
\cline{3-5}& & Act. & Com. & Cou. & \\ \hline
\multicolumn{7}{l}{\emph{Qwen3-VL-4B}} \\ \hline
SeqFT & 7.42 & 47.29 & 48.66 & 44.03 & 46.66 & -13.86 \\
EWC & 4.34 & 40.06 & 40.42 & 38.40 & 39.62 & -18.14 \\
GEM & 8.28 & 47.64 & 42.54 & 41.34 & 43.84 & -12.89 \\
LwF & 26.67 & \textbf{66.97} & 58.19 & 40.89 & 55.35 & -5.74 \\
replay & 20.79 & 61.20 & 60.88 & \textbf{52.27} & 58.11 & -2.72 \\
replay-online & 8.86 & \underline{65.65} & \textbf{69.68} & \underline{50.67} & \textbf{62.00} & \underline{-0.83} \\
SeqLoRA & 32.18 & 38.66 & 45.56 & 23.38 & 35.87 & -1.62 \\
O-LoRA & 5.23 & 40.06 & 48.90 & 37.01 & 41.99 & -1.25 \\
LayerNorm & 23.77 & 60.29 & 59.09 & 43.06 & 54.15 & -1.37 \\
MIGU & 27.44 & 47.64 & 57.46 & 37.29 & 47.46 & -4.87 \\
SPTC-F (ours) & \underline{35.59} & 62.66 & 58.76 & 48.19 & 56.54 & -1.53 \\
SPTC-S (ours) & \textbf{38.74} & 62.15 & \underline{61.53} & 47.50 & 57.06 & \textbf{-0.50} \\
\hline
\multicolumn{7}{l}{\emph{LLaVA-1.5-7B}} \\ \hline
SeqFT  & 10.69 & 41.72 & 39.36 & 43.03 & 41.37 & -26.84 \\
EWC & 21.92 & 46.38 & 52.40 & 24.21 & 41.00 & -10.04 \\
GEM & 24.17 & 49.65 & 53.63 & 30.16 & 44.48 & -7.18 \\
LwF & 36.02 & 67.66 & 58.11 & 2.07 & 42.62 & -0.51 \\
replay & 13.61 & 65.79 & 70.90 & 45.62 & 60.77 & -0.78 \\
replay-online & 10.46 & 67.25 & 69.11 & 44.93 & 60.43 & -1.66 \\
SeqLoRA & 31.04 & \textbf{75.31} & 75.63 & \underline{53.10} & 68.01 & -0.51 \\
O-LoRA & 6.80 & 70.38 & 72.94 & 52.30 & 65.21 & -0.26 \\
LayerNorm & 30.71 & 69.68 & 60.39 & 2.91 & 44.33 & \underline{-0.20} \\
MIGU & 21.81 & 67.66 & 52.40 & 42.89 & 54.32 & -8.62 \\
SPTC-F (ours) & \underline{37.51} & \underline{74.48} & \underline{77.18} & 53.06 & \underline{68.24} & -0.29 \\
SPTC-S (ours) & \textbf{41.94} & \textbf{75.31} & \textbf{77.34} & \textbf{53.27} & \textbf{68.64} & \textbf{-0.16} \\
\hlineB{4}
\end{tabular}}}
\caption{Multimodal Large Models}
\label{tab1}
\end{table}

\textbf{Large Language Model} \\
\textbf{Multimodal Large Models} \\

\subsection{Discussion}
